MicroFlow: Domain-Specific Optical Flow for Ground Deformation Estimation in Seismic Events

Dense ground displacement measurements are crucial for geological studies but are impractical to collect directly. Traditionally, displacement fields are estimated using patch matching on optical satellite images from different acquisition times. While deep learning-based optical flow models are promising, their adoption in ground deformation analysis is hindered by challenges such as the absence of real ground truth, the need for sub-pixel precision, and temporal variations due to geological or anthropogenic changes. In particular, we identify that deep learning models relying on explicit correlation layers struggle at estimating small displacements in real-world conditions. Instead, we propose a model that employs iterative refinements with explicit warping layers and a correlation-independent backbone, enabling sub-pixel precision. Additionally, a non-convex variant of Total Variation regularization preserves fault-line sharpness while maintaining smoothness elsewhere. Our model significantly outperforms widely used geophysics methods on semi-synthetic benchmarks and generalizes well to challenging real-world scenarios captured by both medium- and high-resolution sensors. Project page: https://jbertrand89.github.io/microflow/.

==> fig/04_1_1_profile_first_fault.tex <==
 \begin{tikzpicture}

  \pgfplotstableread{
0 -0.7150237560272217 -0.75 -0.8720703125 -0.76611328125 -0.7490234375 -0.8271484375
1 -0.6996685266494751 -0.737500011920929 -0.86279296875 -0.7451171875 -0.7431640625 -0.8271484375
2 -0.6981809735298157 -0.7333333492279053 -0.85205078125 -0.73974609375 -0.7431640625 -0.8271484375
3 -0.702643871307373 -0.731249988079071 -0.8505859375 -0.78955078125 -0.7431640625 -0.8271484375
4 -0.6810526251792908 -0.699999988079071 -0.837890625 -0.736328125 -0.7431640625 -0.8271484375
5 -0.6949031949043274 -0.6875 -0.82568359375 -0.734375 -0.71875 -0.8271484375
6 -0.711142897605896 -0.6833333373069763 -0.8046875 -0.7099609375 -0.71875 -0.8271484375
7 -0.707228422164917 -0.6812499761581421 -0.79150390625 -0.7158203125 -0.71875 -0.8271484375
8 -0.6829754710197449 -0.6800000071525574 -0.791015625 -0.677734375 -0.66357421875 -0.7646484375
9 -0.6600110530853271 -0.6791666746139526 -0.7705078125 -0.67431640625 -0.66357421875 -0.7646484375
10 -0.6384528875350952 -0.6785714030265808 -0.76708984375 -0.67236328125 -0.66357421875 -0.7646484375
11 -0.623275637626648 -0.6781250238418579 -0.755859375 -0.64892578125 -0.66357421875 -0.7646484375
12 -0.6149672269821167 -0.668749988079071 -0.75927734375 -0.66943359375 -0.66015625 -0.7646484375
13 -0.5948641300201416 -0.65625 -0.74755859375 -0.6220703125 -0.66015625 -0.7646484375
14 -0.589820384979248 -0.643750011920929 -0.75 -0.626953125 -0.66015625 -0.7646484375
15 -0.5866679549217224 -0.6312500238418579 -0.7431640625 -0.62548828125 -0.66015625 -0.7646484375
16 -0.5852924585342407 -0.5749849677085876 -0.74072265625 -0.625 -0.66015625 -0.7646484375
17 -0.5931355357170105 -0.5749849677085876 -0.7138671875 -0.65380859375 -0.66015625 -0.7646484375
18 -0.5955238342285156 -0.5749849677085876 -0.7177734375 -0.60400390625 -0.66015625 -0.7646484375
19 -0.603447675704956 -0.5749849677085876 -0.70849609375 -0.654296875 -0.66015625 -0.7646484375
20 -0.6097583770751953 -0.5749849677085876 -0.6884765625 -0.6875 -0.66015625 -0.7646484375
21 -0.6163440942764282 -0.5749849677085876 -0.67724609375 -0.67138671875 -0.66015625 -0.7646484375
22 -0.6220482587814331 -0.5749849677085876 -0.68310546875 -0.68359375 -0.66015625 -0.7646484375
23 -0.6314821243286133 -0.5749849677085876 -0.689453125 -0.685546875 -0.66015625 -0.7646484375
24 -0.6452540159225464 -0.6750749945640564 -0.685546875 -0.68896484375 -0.66015625 -0.7646484375
25 -0.6534233689308167 -0.6751700043678284 -0.6669921875 -0.67138671875 -0.66015625 -0.7646484375
26 -0.6503350734710693 -0.6751700043678284 -0.68310546875 -0.650390625 -0.66015625 -0.7646484375
27 -0.6486492156982422 -0.6750749945640564 -0.7021484375 -0.685546875 -0.66015625 -0.7646484375
28 -0.6620281338691711 -0.671875 -0.73681640625 -0.65380859375 -0.66015625 -0.76025390625
29 -0.6737852096557617 -0.671875 -0.71728515625 -0.67529296875 -0.66015625 -0.76025390625
30 -0.6733993291854858 -0.671875 -0.7373046875 -0.677734375 -0.66015625 -0.76025390625
31 -0.6713674664497375 -0.671875 -0.73046875 -0.677734375 -0.66015625 -0.76025390625
32 -0.6700491905212402 -0.6691176295280457 -0.73193359375 -0.6787109375 -0.66015625 -0.76025390625
33 -0.6590025424957275 -0.6644736528396606 -0.72119140625 -0.62939453125 -0.646484375 -0.76025390625
34 -0.6526944637298584 -0.6607142686843872 -0.72021484375 -0.63671875 -0.646484375 -0.76025390625
35 -0.642223060131073 -0.657608687877655 -0.72412109375 -0.65087890625 -0.646484375 -0.76025390625
36 -0.644623875617981 -0.6557692289352417 -0.75341796875 -0.64892578125 -0.646484375 -0.76025390625
37 -0.6428014039993286 -0.6543103456497192 -0.74658203125 -0.6494140625 -0.6201171875 -0.76025390625
38 -0.6417409777641296 -0.653124988079071 -0.74169921875 -0.63720703125 -0.6201171875 -0.76025390625
39 -0.6411306858062744 -0.6546875238418579 -0.7548828125 -0.654296875 -0.6201171875 -0.76025390625
40 -0.6369256377220154 -0.6572580933570862 -0.78125 -0.6044921875 -0.6201171875 -0.76025390625
41 -0.6322968006134033 -0.6588709950447083 -0.7607421875 -0.64208984375 -0.6201171875 -0.76025390625
42 -0.6211961507797241 -0.6604838967323303 -0.76220703125 -0.626953125 -0.6201171875 -0.76025390625
43 -0.6174879670143127 -0.6620967984199524 -0.76416015625 -0.64111328125 -0.6201171875 -0.76025390625
44 -0.6238325238227844 -0.6640625 -0.783203125 -0.603515625 -0.6201171875 -0.76025390625
45 -0.623350977897644 -0.6647058725357056 -0.7841796875 -0.5771484375 -0.5908203125 -0.76025390625
46 -0.6276111602783203 -0.6652777791023254 -0.7822265625 -0.55517578125 -0.5908203125 -0.76025390625
47 -0.6342344880104065 -0.6657894849777222 -0.783203125 -0.57275390625 -0.5908203125 -0.76025390625
48 -0.6325522661209106 -0.6662499904632568 -0.77734375 -0.52880859375 -0.5908203125 -0.76025390625
49 -0.6469097137451172 -0.668749988079071 -0.76171875 -0.5244140625 -0.5908203125 -0.76025390625
50 -0.6626629829406738 -0.6712499856948853 -0.7705078125 -0.58837890625 -0.5908203125 -0.76025390625
51 -0.6718114614486694 -0.6737500429153442 -0.7490234375 -0.54248046875 -0.5908203125 -0.76025390625
52 -0.6715447902679443 -0.6791666746139526 -0.751953125 -0.564453125 -0.5908203125 -0.76025390625
53 -0.669618546962738 -0.6865384578704834 -0.7333984375 -0.53759765625 -0.5908203125 -0.76025390625
54 -0.6792826652526855 -0.6928571462631226 -0.7392578125 -0.5576171875 -0.5908203125 -0.76025390625
55 -0.6753865480422974 -0.6983333230018616 -0.73388671875 -0.58251953125 -0.5908203125 -0.76025390625
56 -0.680863618850708 -0.7016667127609253 -0.76904296875 -0.6259765625 -0.5908203125 -0.7333984375
57 -0.6812391877174377 -0.703125 -0.7412109375 -0.55810546875 -0.5908203125 -0.7333984375
58 -0.678508460521698 -0.7044117450714111 -0.763671875 -0.619140625 -0.625 -0.7333984375
59 -0.6801761388778687 -0.7055555582046509 -0.748046875 -0.64453125 -0.625 -0.7333984375
60 -0.6785104274749756 -0.7074999809265137 -0.767578125 -0.6298828125 -0.625 -0.7333984375
61 -0.6790096759796143 -0.7074999809265137 -0.74951171875 -0.6494140625 -0.625 -0.7333984375
62 -0.6875951290130615 -0.7055555582046509 -0.75244140625 -0.6318359375 -0.625 -0.7333984375
63 -0.6997037529945374 -0.703125 -0.7607421875 -0.66845703125 -0.625 -0.7333984375
64 -0.7091358304023743 -0.699999988079071 -0.7451171875 -0.68798828125 -0.625 -0.7333984375
65 -0.707062840461731 -0.6958333253860474 -0.7275390625 -0.66845703125 -0.625 -0.7333984375
66 -0.695715606212616 -0.6899999976158142 -0.73974609375 -0.642578125 -0.625 -0.7333984375
67 -0.6876654624938965 -0.6812499761581421 -0.73291015625 -0.64794921875 -0.625 -0.7333984375
68 -0.6764835119247437 -0.6699999570846558 -0.705078125 -0.6435546875 -0.625 -0.68115234375
69 -0.6744721531867981 -0.6625000238418579 -0.67919921875 -0.66259765625 -0.625 -0.63623046875
70 -0.6601534485816956 -0.6596153974533081 -0.67333984375 -0.662109375 -0.625 -0.63623046875
71 -0.6491844058036804 -0.6659091114997864 -0.67333984375 -0.634765625 -0.625 -0.63623046875
72 -0.6422209739685059 -0.6704545617103577 -0.66552734375 -0.7294921875 -0.625 -0.63623046875
73 -0.6347928643226624 -0.6711538434028625 -0.63525390625 -0.67529296875 -0.625 -0.63623046875
74 -0.6386294364929199 -0.67166668176651 -0.67431640625 -0.63232421875 -0.60791015625 -0.63623046875
75 -0.6384042501449585 -0.6720588207244873 -0.642578125 -0.63427734375 -0.60791015625 -0.63623046875
76 -0.631842851638794 -0.671875 -0.63623046875 -0.599609375 -0.60791015625 -0.62646484375
77 -0.6363005638122559 -0.6714285612106323 -0.62646484375 -0.6064453125 -0.60791015625 -0.62646484375
78 -0.6390402317047119 -0.6708333492279053 -0.64501953125 -0.6005859375 -0.60791015625 -0.62646484375
79 -0.635231614112854 -0.6699999570846558 -0.63720703125 -0.62890625 -0.60791015625 -0.62646484375
80 -0.6169317960739136 -0.668749988079071 -0.65185546875 -0.6025390625 -0.60791015625 -0.62646484375
81 -0.6108905673027039 -0.6666666269302368 -0.63330078125 -0.63525390625 -0.60791015625 -0.62646484375
82 -0.600452721118927 -0.6625000238418579 -0.62841796875 -0.59033203125 -0.60791015625 -0.62646484375
83 -0.5861849188804626 -0.6499999761581421 -0.6123046875 -0.6064453125 -0.60791015625 -0.62646484375
84 -0.5613469481468201 -0.6187499761581421 -0.591796875 -0.5859375 -0.6005859375 -0.61474609375
85 -0.5346691012382507 -0.606249988079071 -0.576171875 -0.5712890625 -0.6005859375 -0.61474609375
86 -0.5208874940872192 -0.59375 -0.5771484375 -0.5693359375 -0.59765625 -0.61474609375
87 -0.48774611949920654 -0.581250011920929 -0.57177734375 -0.5625 -0.59765625 -0.61474609375
88 -0.4646538496017456 -0.26875001192092896 -0.5537109375 -0.52685546875 -0.53125 -0.60302734375
89 -0.4323580265045166 -0.2666666805744171 -0.51611328125 -0.56591796875 -0.53125 -0.490966796875
90 -0.35747355222702026 -0.26249998807907104 -0.498046875 -0.498291015625 -0.53125 -0.490966796875
91 -0.3010448217391968 -0.25 -0.4912109375 -0.52001953125 -0.53125 -0.490966796875
92 -0.2370086908340454 0.0 -0.46923828125 -0.437744140625 -0.4345703125 -0.490478515625
93 -0.16866666078567505 0.012500000186264515 -0.485107421875 -0.423095703125 -0.423095703125 -0.4638671875
94 -0.09063899517059326 0.01666666753590107 -0.423828125 -0.337158203125 -0.367919921875 -0.4638671875
95 -0.05198538303375244 0.01875000074505806 -0.408935546875 -0.31396484375 -0.322509765625 -0.4638671875
96 0.03447425365447998 0.4312500059604645 -0.303955078125 -0.1041259765625 -0.1044921875 -0.28955078125
97 0.1383417844772339 0.4333333373069763 -0.303955078125 -0.0271453857421875 -0.0287628173828125 -0.28564453125
98 0.32110774517059326 0.4375 -0.1490478515625 0.322998046875 0.32275390625 -0.17626953125
99 1.8089263439178467 0.44999998807907104 0.0963134765625 0.483154296875 0.483154296875 0.0924072265625
100 1.0005769729614258 0.8812500238418579 0.59423828125 0.73681640625 0.73876953125 0.59375
101 1.2202928066253662 0.893750011920929 0.94921875 0.98974609375 0.99169921875 0.94921875
102 1.4163954257965088 0.90625 1.4345703125 1.107421875 1.1171875 1.44140625
103 1.4605154991149902 0.918749988079071 1.63671875 1.2314453125 1.23046875 1.615234375
104 1.5023313760757446 1.28125 1.7822265625 1.328125 1.333984375 1.740234375
105 1.555227279663086 1.2833333015441895 1.8447265625 1.4912109375 1.51171875 1.736328125
106 1.571997046470642 1.287500023841858 1.794921875 1.4599609375 1.541015625 1.736328125
107 1.6010243892669678 1.2999999523162842 1.8115234375 1.58984375 1.55078125 1.736328125
108 1.636757731437683 1.649999976158142 1.6748046875 1.6875 1.705078125 1.6669921875
109 1.6710013151168823 1.662500023841858 1.65625 1.69921875 1.72265625 1.6611328125
110 1.6914255619049072 1.6666666269302368 1.64453125 1.7119140625 1.72265625 1.6611328125
111 1.7032853364944458 1.6687500476837158 1.6591796875 1.7138671875 1.72265625 1.6611328125
112 1.7219619750976562 1.7000000476837158 1.6416015625 1.7607421875 1.7607421875 1.6611328125
113 1.733129858970642 1.712499976158142 1.6474609375 1.763671875 1.7841796875 1.6611328125
114 1.742017388343811 1.741666555404663 1.6259765625 1.74609375 1.7841796875 1.6611328125
115 1.7458362579345703 1.7464284896850586 1.6572265625 1.794921875 1.7841796875 1.6611328125
116 1.7484995126724243 1.7477271556854248 1.6982421875 1.7880859375 1.7841796875 1.685546875
117 1.7504215240478516 1.7483333349227905 1.6533203125 1.794921875 1.7841796875 1.685546875
118 1.749605655670166 1.7486841678619385 1.6689453125 1.7861328125 1.7841796875 1.685546875
119 1.7511539459228516 1.748913049697876 1.6875 1.7822265625 1.7841796875 1.685546875
120 1.7530092000961304 1.7490739822387695 1.6884765625 1.7998046875 1.7841796875 1.685546875
121 1.757533311843872 1.749193549156189 1.66796875 1.8671875 1.8076171875 1.685546875
122 1.7644705772399902 1.751562476158142 1.65625 1.771484375 1.8115234375 1.685546875
123 1.7649270296096802 1.7529411315917969 1.6962890625 1.798828125 1.8115234375 1.685546875
124 1.7779498100280762 1.754166603088379 1.6826171875 1.8173828125 1.8115234375 1.685546875
125 1.7851496934890747 1.755263090133667 1.6728515625 1.79296875 1.8115234375 1.685546875
126 1.7855348587036133 1.7554877996444702 1.66796875 1.8095703125 1.8115234375 1.685546875
127 1.7888331413269043 1.7556817531585693 1.701171875 1.8125 1.8115234375 1.685546875
128 1.7836101055145264 1.7579545974731445 1.6982421875 1.8125 1.8115234375 1.685546875
129 1.7813867330551147 1.7602272033691406 1.6943359375 1.82421875 1.8115234375 1.685546875
130 1.7835110425949097 1.7625000476837158 1.7041015625 1.8515625 1.8115234375 1.685546875
131 1.7839157581329346 1.763888955116272 1.7109375 1.84375 1.8115234375 1.685546875
132 1.7873409986495972 1.7652174234390259 1.70703125 1.84375 1.8115234375 1.685546875
133 1.7833375930786133 1.7664893865585327 1.6982421875 1.8154296875 1.8115234375 1.685546875
134 1.7852743864059448 1.767708420753479 1.6845703125 1.806640625 1.8115234375 1.685546875
135 1.7924693822860718 1.769791603088379 1.6787109375 1.8408203125 1.8125 1.685546875
136 1.7945506572723389 1.771875023841858 1.6884765625 1.8212890625 1.8125 1.685546875
137 1.7946466207504272 1.773958444595337 1.671875 1.8369140625 1.8125 1.685546875
138 1.8069207668304443 1.7781250476837158 1.681640625 1.8388671875 1.8125 1.685546875
139 1.8074181079864502 1.7785714864730835 1.7001953125 1.8466796875 1.8125 1.685546875
140 1.8225023746490479 1.779166579246521 1.6923828125 1.865234375 1.8125 1.685546875
141 1.8281054496765137 1.7799999713897705 1.666015625 1.8671875 1.8125 1.685546875
142 1.8278734683990479 1.7861111164093018 1.66015625 1.8310546875 1.8125 1.685546875
143 1.836482048034668 1.7972221374511719 1.6845703125 1.8173828125 1.8125 1.685546875
144 1.835799217224121 1.808333396911621 1.689453125 1.796875 1.8125 1.685546875
145 1.8269115686416626 1.8194444179534912 1.693359375 1.828125 1.8125 1.685546875
146 1.8207283020019531 1.8273149728775024 1.701171875 1.8359375 1.8125 1.685546875
147 1.8157728910446167 1.8273149728775024 1.7177734375 1.8369140625 1.8125 1.685546875
148 1.8002270460128784 1.8273149728775024 1.697265625 1.8251953125 1.8125 1.685546875
149 1.814632534980774 1.8273149728775024 1.68359375 1.8310546875 1.8125 1.685546875
150 1.8069862127304077 1.8223683834075928 1.6650390625 1.84765625 1.8125 1.685546875
151 1.79542875289917 1.8184782266616821 1.7060546875 1.8115234375 1.8125 1.685546875
152 1.7917745113372803 1.8157408237457275 1.70703125 1.7919921875 1.8125 1.685546875
153 1.7863030433654785 1.8137096166610718 1.6962890625 1.798828125 1.8125 1.685546875
154 1.7922247648239136 1.814062476158142 1.6962890625 1.83203125 1.8125 1.685546875
155 1.7965232133865356 1.814062476158142 1.712890625 1.80859375 1.8125 1.685546875
156 1.7990233898162842 1.814062476158142 1.6845703125 1.798828125 1.8125 1.685546875
157 1.7969733476638794 1.814062476158142 1.67578125 1.8369140625 1.8125 1.6904296875
158 1.8036479949951172 1.8120968341827393 1.673828125 1.8046875 1.806640625 1.6904296875
159 1.8080278635025024 1.8100000619888306 1.6845703125 1.830078125 1.806640625 1.6904296875
160 1.8158034086227417 1.8077586889266968 1.66796875 1.8115234375 1.806640625 1.6904296875
161 1.8166804313659668 1.8053572177886963 1.6796875 1.7998046875 1.806640625 1.6904296875
162 1.8056564331054688 1.8017857074737549 1.662109375 1.7548828125 1.806640625 1.6904296875
163 1.8060756921768188 1.798214316368103 1.6748046875 1.8037109375 1.806640625 1.6904296875
164 1.8121540546417236 1.7961537837982178 1.6669921875 1.7763671875 1.806640625 1.6904296875
165 1.7937897443771362 1.7937500476837158 1.6630859375 1.7978515625 1.806640625 1.6904296875
166 1.7904144525527954 1.7909090518951416 1.6591796875 1.7783203125 1.806640625 1.6904296875
167 1.7859933376312256 1.787500023841858 1.666015625 1.8193359375 1.806640625 1.6904296875
168 1.7853643894195557 1.783333420753479 1.6796875 1.798828125 1.806640625 1.6904296875
169 1.775247573852539 1.7781250476837158 1.65625 1.8046875 1.806640625 1.6904296875
170 1.7772960662841797 1.774920105934143 1.646484375 1.794921875 1.806640625 1.6904296875
171 1.7720741033554077 1.774785041809082 1.6650390625 1.80078125 1.806640625 1.6904296875
172 1.777858853340149 1.7746798992156982 1.66796875 1.83203125 1.806640625 1.6904296875
173 1.7765133380889893 1.774614930152893 1.6630859375 1.8154296875 1.806640625 1.6904296875
174 1.7709420919418335 1.774614930152893 1.66796875 1.8154296875 1.806640625 1.6904296875
175 1.7757195234298706 1.774614930152893 1.6875 1.7841796875 1.806640625 1.6904296875
176 1.7686079740524292 1.774614930152893 1.7119140625 1.783203125 1.806640625 1.6904296875
177 1.7599159479141235 1.774614930152893 1.677734375 1.8115234375 1.806640625 1.6904296875
178 1.753046989440918 1.774614930152893 1.67578125 1.7900390625 1.806640625 1.693359375
179 1.7521686553955078 1.774614930152893 1.6904296875 1.794921875 1.806640625 1.693359375
180 1.7456730604171753 1.774614930152893 1.67578125 1.82421875 1.806640625 1.693359375
181 1.7382910251617432 1.774614930152893 1.6943359375 1.8203125 1.806640625 1.693359375
182 1.7461934089660645 1.774614930152893 1.6962890625 1.791015625 1.806640625 1.693359375
183 1.7514303922653198 1.774614930152893 1.697265625 1.7861328125 1.814453125 1.693359375
184 1.7531471252441406 1.774614930152893 1.720703125 1.80078125 1.814453125 1.693359375
185 1.7596608400344849 1.774614930152893 1.712890625 1.8408203125 1.814453125 1.6962890625
186 1.7693573236465454 1.774614930152893 1.7138671875 1.8349609375 1.814453125 1.6962890625
187 1.7731999158859253 1.774614930152893 1.7275390625 1.8095703125 1.82421875 1.6962890625
188 1.76948881149292 1.774614930152893 1.7197265625 1.8046875 1.82421875 1.6962890625
189 1.7805540561676025 1.774614930152893 1.7001953125 1.791015625 1.82421875 1.6962890625
190 1.7807871103286743 1.774614930152893 1.7060546875 1.8076171875 1.82421875 1.6962890625
191 1.7827353477478027 1.774614930152893 1.7060546875 1.7998046875 1.82421875 1.6962890625
192 1.7885448932647705 1.774614930152893 1.689453125 1.8154296875 1.82421875 1.6962890625
193 1.7808839082717896 1.774614930152893 1.6748046875 1.828125 1.82421875 1.6962890625
194 1.7799676656723022 1.774595022201538 1.67578125 1.8603515625 1.82421875 1.6962890625
195 1.771289587020874 1.7745800018310547 1.6884765625 1.8388671875 1.82421875 1.6962890625
196 1.7712898254394531 1.7745800018310547 1.677734375 1.849609375 1.82421875 1.6962890625
197 1.7510803937911987 1.774595022201538 1.6640625 1.8505859375 1.833984375 1.6962890625
198 1.746856689453125 1.774614930152893 1.6640625 1.84375 1.833984375 1.6962890625
199 1.7430332899093628 1.774614930152893 1.673828125 1.826171875 1.833984375 1.6962890625
      }{\testdatanorm}

    \begin{axis}[
        width=5cm,
        height=4cm,
        xmax=130,xmin=70,
        ymax=2,ymin=-1,
        % ymax=2.5,ymin=-1.8,
        ytick={-2,-1.5,-1, -0.5,0,0.5,1, 1.5, 2, 2.5},
        xlabel = {\small Distance along profile (m)}, 
        % grid=both,
        ylabel={\small\parbox{4cm}{Displacement in the \\ North/South direction (m)}},   
        y label style={yshift=-7pt},  
        legend columns=4,
        legend style={
            % cells={anchor=west},
            at={(1.25,1.4)},
            anchor=north,
            % only marks,
            /tikz/every even column/.append style={column sep=0.5cm}
            },
        ]        
         \addplot [color=blue, line width=1.3, opacity=1] table [x expr={\thisrowno{0}},y expr={\thisrowno{1}}] {\testdatanorm};
        \addplot [color=cyan, line width=1.3, opacity=1] table [x expr={\thisrowno{0}},y expr={\thisrowno{2}}] {\testdatanorm};
        \addplot [color=gray, line width=1.3, opacity=1] table [x expr={\thisrowno{0}},y expr={\thisrowno{3}}] {\testdatanorm};
        \addplot [color=red, line width=1.3, opacity=1] table [x expr={\thisrowno{0}},y expr={\thisrowno{5}}] {\testdatanorm};
        \legend{\cosicorr, \micmac, \gfn, Ours},
    \end{axis}
\end{tikzpicture}

==> fig/04_1_2_profile_second_fault.tex <==
\begin{tikzpicture}

  \pgfplotstableread{
0 1.842961311340332 1.819117784500122 1.8134765625 1.8173828125 1.82421875 1.7998046875
1 1.8374253511428833 1.822058916091919 1.7783203125 1.83203125 1.82421875 1.796875
2 1.8556559085845947 1.8235714435577393 1.7685546875 1.8505859375 1.82421875 1.796875
3 1.85257089138031 1.8236486911773682 1.77734375 1.8740234375 1.82421875 1.796875
4 1.8530833721160889 1.8237178325653076 1.787109375 1.8525390625 1.82421875 1.796875
5 1.855975866317749 1.8237804174423218 1.802734375 1.87890625 1.82421875 1.796875
6 1.8588955402374268 1.8277778625488281 1.837890625 1.8720703125 1.8505859375 1.8330078125
7 1.8624625205993652 1.8325001001358032 1.8564453125 1.9189453125 1.8623046875 1.8330078125
8 1.8532626628875732 1.8363635540008545 1.875 1.947265625 1.900390625 1.8330078125
9 1.7924039363861084 1.839583396911621 1.8642578125 1.90625 1.900390625 1.8330078125
10 1.8410812616348267 1.840999960899353 1.876953125 1.90234375 1.900390625 1.8330078125
11 1.9238004684448242 1.838043451309204 1.875 1.9228515625 1.900390625 1.8330078125
12 1.9140348434448242 1.8345237970352173 1.9169921875 1.935546875 1.900390625 1.8330078125
13 1.8199830055236816 1.8302631378173828 1.916015625 1.935546875 1.900390625 1.8330078125
14 1.8449997901916504 1.8276315927505493 1.939453125 1.908203125 1.900390625 1.8427734375
15 1.8114843368530273 1.827380895614624 1.9365234375 1.88671875 1.900390625 1.8427734375
16 1.794898271560669 1.8271739482879639 1.93359375 1.900390625 1.900390625 1.8427734375
17 1.7919496297836304 1.8270833492279053 1.8671875 1.95703125 1.9208984375 1.8427734375
18 1.7955838441848755 1.824305534362793 1.84765625 1.912109375 1.9208984375 1.8427734375
19 1.8035610914230347 1.8242957592010498 1.83984375 1.931640625 1.9208984375 1.8427734375
20 1.8158185482025146 1.8242857456207275 1.8037109375 1.912109375 1.908203125 1.8427734375
21 1.8211264610290527 1.8242647647857666 1.78515625 1.93359375 1.890625 1.8427734375
22 1.826727271080017 1.8268518447875977 1.7783203125 1.8583984375 1.8828125 1.8427734375
23 1.8127167224884033 1.8267240524291992 1.7978515625 1.884765625 1.8828125 1.8427734375
24 1.8055765628814697 1.8266128301620483 1.8095703125 1.7861328125 1.8056640625 1.8427734375
25 1.8067967891693115 1.8265151977539062 1.783203125 1.77734375 1.7841796875 1.8427734375
26 1.8100043535232544 1.8241071701049805 1.7705078125 1.8310546875 1.7841796875 1.8427734375
27 1.8176746368408203 1.8223215341567993 1.7978515625 1.7998046875 1.76953125 1.8427734375
28 1.8075628280639648 1.820535659790039 1.8427734375 1.728515625 1.75390625 1.8427734375
29 1.7988489866256714 1.818750023841858 1.8203125 1.74609375 1.75390625 1.8701171875
30 1.7917242050170898 1.8169643878936768 1.8134765625 1.708984375 1.75390625 1.8701171875
31 1.7909214496612549 1.8151785135269165 1.8115234375 1.76171875 1.75390625 1.8876953125
32 1.7859914302825928 1.8133928775787354 1.82421875 1.69140625 1.75390625 1.8876953125
33 1.7894736528396606 1.8116071224212646 1.81640625 1.701171875 1.75390625 1.8876953125
34 1.7787271738052368 1.8111110925674438 1.86328125 1.703125 1.75390625 1.8876953125
35 1.781191349029541 1.8105770349502563 1.865234375 1.7392578125 1.75390625 1.8876953125
36 1.7801378965377808 1.8100000619888306 1.849609375 1.6845703125 1.75390625 1.8876953125
37 1.7826334238052368 1.8093750476837158 1.822265625 1.7158203125 1.75390625 1.841796875
38 1.7886922359466553 1.8086955547332764 1.8271484375 1.7138671875 1.767578125 1.841796875
39 1.7905151844024658 1.8079545497894287 1.8447265625 1.736328125 1.76953125 1.841796875
40 1.7852723598480225 1.8071428537368774 1.822265625 1.75 1.76953125 1.841796875
41 1.7837285995483398 1.806249976158142 1.7880859375 1.7578125 1.76953125 1.841796875
42 1.78412926197052 1.8052631616592407 1.78515625 1.7880859375 1.7724609375 1.841796875
43 1.782131552696228 1.804729700088501 1.8359375 1.8359375 1.7724609375 1.841796875
44 1.790451169013977 1.804166555404663 1.8779296875 1.763671875 1.7724609375 1.888671875
45 1.792422890663147 1.8035714626312256 1.8486328125 1.7744140625 1.7724609375 1.888671875
46 1.790795922279358 1.802142858505249 1.8759765625 1.7890625 1.7724609375 1.888671875
47 1.7995471954345703 1.8007142543792725 1.9072265625 1.7861328125 1.7724609375 1.9130859375
48 1.7985576391220093 1.7999999523162842 1.9111328125 1.7431640625 1.7724609375 1.9130859375
49 1.7928403615951538 1.799242377281189 1.8916015625 1.765625 1.7724609375 1.9130859375
50 1.7881278991699219 1.798437476158142 1.8935546875 1.806640625 1.7724609375 1.9130859375
51 1.7923673391342163 1.798437476158142 1.939453125 1.8583984375 1.826171875 1.9130859375
52 1.7944018840789795 1.7991936206817627 1.9462890625 1.8359375 1.826171875 1.9130859375
53 1.816049575805664 1.8008620738983154 1.9228515625 1.87109375 1.875 1.9130859375
54 1.8242011070251465 1.8017857074737549 1.93359375 1.912109375 1.912109375 1.9130859375
55 1.8289494514465332 1.8009999990463257 1.9794921875 1.89453125 1.912109375 1.9130859375
56 1.8478752374649048 1.7999999523162842 1.9677734375 1.8193359375 1.880859375 1.9130859375
57 1.8467639684677124 1.7986841201782227 1.94140625 1.8779296875 1.880859375 1.9130859375
58 1.8215656280517578 1.796875 1.9423828125 1.912109375 1.896484375 1.9130859375
59 1.845224142074585 1.7928571701049805 1.9755859375 1.908203125 1.9140625 1.9130859375
60 1.8574965000152588 1.787500023841858 1.990234375 1.9873046875 1.9912109375 1.9619140625
61 1.8859083652496338 1.7805554866790771 1.9638671875 1.9873046875 1.9912109375 1.9951171875
62 1.8914904594421387 1.7645848989486694 1.966796875 2.08203125 2.046875 1.9951171875
63 1.9242043495178223 1.756250023841858 1.9951171875 2.0 2.03125 1.9951171875
64 1.9631011486053467 1.756250023841858 2.015625 2.064453125 2.05859375 1.9951171875
65 1.9880266189575195 1.7645848989486694 1.994140625 2.05859375 2.060546875 1.9951171875
66 2.0503017902374268 2.049999952316284 2.017578125 2.103515625 2.107421875 1.9951171875
67 2.1174919605255127 2.0625 2.037109375 2.111328125 2.109375 1.9951171875
68 2.1705126762390137 2.066666603088379 2.076171875 2.205078125 2.201171875 2.037109375
69 2.199936628341675 2.0687499046325684 2.052734375 2.173828125 2.20703125 2.087890625
70 2.242438554763794 2.25 2.080078125 2.212890625 2.22265625 2.087890625
71 2.2840898036956787 2.262500047683716 2.099609375 2.236328125 2.25390625 2.087890625
72 2.324982166290283 2.2666666507720947 2.0546875 2.31640625 2.31640625 2.087890625
73 2.3337185382843018 2.268749952316284 2.03515625 2.267578125 2.31640625 2.03125
74 2.328047275543213 2.269444465637207 2.05078125 2.3046875 2.318359375 2.03125
75 2.353954792022705 2.2699999809265137 2.068359375 2.2734375 2.326171875 2.03125
76 2.3604607582092285 2.2704546451568604 2.05078125 2.302734375 2.326171875 2.03125
77 2.3460633754730225 2.2708334922790527 2.029296875 2.27734375 2.326171875 2.03125
78 2.3523142337799072 2.2714285850524902 2.041015625 2.291015625 2.326171875 2.03125
79 2.3550193309783936 2.2718749046325684 2.056640625 2.326171875 2.34765625 2.03125
80 2.372270345687866 2.2722220420837402 2.052734375 2.328125 2.34765625 2.03125
81 2.3758180141448975 2.2725000381469727 2.033203125 2.361328125 2.34765625 2.03125
82 2.387343406677246 2.377500057220459 2.048828125 2.34765625 2.34765625 2.03125
83 2.3927268981933594 2.3821427822113037 2.0859375 2.37109375 2.34765625 2.115234375
84 2.380964994430542 2.3863635063171387 2.08984375 2.353515625 2.34765625 2.115234375
85 2.3787262439727783 2.3902173042297363 2.0703125 2.33984375 2.34765625 2.115234375
86 2.37565016746521 2.393749952316284 2.087890625 2.32421875 2.34765625 2.115234375
87 2.373084545135498 2.3961539268493652 2.099609375 2.3359375 2.34765625 2.115234375
88 2.3675711154937744 2.3961539268493652 2.130859375 2.3046875 2.34765625 2.138671875
89 2.362544298171997 2.3949999809265137 2.134765625 2.34765625 2.34765625 2.162109375
90 2.360024929046631 2.3930001258850098 2.130859375 2.34375 2.34765625 2.162109375
91 2.3596794605255127 2.392307758331299 2.146484375 2.32421875 2.34765625 2.1953125
92 2.355564832687378 2.393749952316284 2.1640625 2.34765625 2.34765625 2.1953125
93 2.348331928253174 2.3954546451568604 2.177734375 2.365234375 2.34765625 2.1953125
94 2.35452938079834 2.3975000381469727 2.177734375 2.341796875 2.34765625 2.1953125
95 2.3538978099823 2.398684024810791 2.193359375 2.318359375 2.34765625 2.1953125
96 2.3571982383728027 2.4000000953674316 2.185546875 2.275390625 2.34765625 2.1953125
97 2.358330249786377 2.40147066116333 2.2265625 2.373046875 2.34765625 2.1953125
98 2.359710454940796 2.404411792755127 2.18359375 2.34375 2.34765625 2.1953125
99 2.357712745666504 2.405555486679077 2.22265625 2.306640625 2.34765625 2.1953125
100 2.3553237915039062 2.40657901763916 2.197265625 2.302734375 2.34765625 2.1953125
101 2.3525235652923584 2.4075000286102295 2.212890625 2.322265625 2.34765625 2.1953125
102 2.346757411956787 2.4083333015441895 2.1953125 2.322265625 2.34765625 2.1953125
103 2.350203275680542 2.409782648086548 2.1953125 2.302734375 2.34765625 2.1953125
104 2.3700664043426514 2.4110000133514404 2.1875 2.28125 2.34765625 2.1953125
105 2.3884494304656982 2.4120371341705322 2.1953125 2.30859375 2.34765625 2.1953125
106 2.3941545486450195 2.4116666316986084 2.185546875 2.296875 2.34765625 2.1953125
107 2.3920722007751465 2.4113636016845703 2.197265625 2.333984375 2.34765625 2.1953125
108 2.386826276779175 2.4111111164093018 2.166015625 2.353515625 2.34765625 2.1953125
109 2.373473644256592 2.41013503074646 2.15625 2.3046875 2.34765625 2.1953125
110 2.3629257678985596 2.4078946113586426 2.1328125 2.310546875 2.34765625 2.1953125
111 2.354583978652954 2.405769109725952 2.171875 2.310546875 2.34765625 2.1953125
112 2.351609230041504 2.403749942779541 2.169921875 2.345703125 2.34765625 2.1953125
113 2.357908248901367 2.403205156326294 2.1796875 2.34375 2.3984375 2.1953125
114 2.35481595993042 2.403571605682373 2.166015625 2.369140625 2.3984375 2.1953125
115 2.3515477180480957 2.4040322303771973 2.19921875 2.3671875 2.3984375 2.1953125
116 2.3441033363342285 2.404629707336426 2.158203125 2.33984375 2.3984375 2.1953125
117 2.345057249069214 2.4054348468780518 2.1640625 2.361328125 2.3984375 2.1953125
118 2.349376678466797 2.4075000286102295 2.1484375 2.361328125 2.3984375 2.1953125
119 2.358144760131836 2.4102940559387207 2.1875 2.34765625 2.3984375 2.1953125
120 2.3667171001434326 2.414285659790039 2.158203125 2.330078125 2.3984375 2.1953125
121 2.372136354446411 2.420454502105713 2.18359375 2.380859375 2.3984375 2.1953125
122 2.384190559387207 2.4276649951934814 2.169921875 2.4140625 2.3984375 2.1953125
123 2.4002952575683594 2.4276649951934814 2.201171875 2.345703125 2.3984375 2.1953125
124 2.4129745960235596 2.4276649951934814 2.1953125 2.4140625 2.3984375 2.1953125
125 2.416672706604004 2.4276649951934814 2.212890625 2.396484375 2.3984375 2.1953125
126 2.4195573329925537 2.4276649951934814 2.2109375 2.40625 2.3984375 2.216796875
127 2.4288649559020996 2.4276649951934814 2.236328125 2.40234375 2.3984375 2.216796875
128 2.426314353942871 2.4276649951934814 2.203125 2.423828125 2.3984375 2.216796875
129 2.4277358055114746 2.4276649951934814 2.220703125 2.39453125 2.3984375 2.216796875
130 2.429600238800049 2.4301350116729736 2.2109375 2.44140625 2.3984375 2.216796875
131 2.4241957664489746 2.4344849586486816 2.22265625 2.408203125 2.3984375 2.216796875
132 2.424865961074829 2.4344849586486816 2.169921875 2.416015625 2.3984375 2.216796875
133 2.4307701587677 2.4301350116729736 2.17578125 2.421875 2.3984375 2.216796875
134 2.4317519664764404 2.4276649951934814 2.181640625 2.412109375 2.3984375 2.216796875
135 2.4339795112609863 2.4276649951934814 2.1953125 2.421875 2.3984375 2.216796875
136 2.429208517074585 2.4276649951934814 2.19140625 2.4140625 2.3984375 2.216796875
137 2.4329071044921875 2.4276649951934814 2.189453125 2.40625 2.3984375 2.216796875
138 2.4322829246520996 2.4276649951934814 2.169921875 2.412109375 2.3984375 2.216796875
139 2.438992500305176 2.4276649951934814 2.1953125 2.41796875 2.3984375 2.216796875
140 2.4235610961914062 2.4276649951934814 2.171875 2.40625 2.3984375 2.216796875
141 2.4145379066467285 2.4276649951934814 2.1796875 2.439453125 2.3984375 2.216796875
142 2.4165151119232178 2.4194445610046387 2.158203125 2.3828125 2.3984375 2.216796875
143 2.416799306869507 2.4083333015441895 2.1875 2.404296875 2.3984375 2.216796875
144 2.4166698455810547 2.3972220420837402 2.197265625 2.3671875 2.3984375 2.216796875
145 2.4233624935150146 2.38611102104187 2.18359375 2.39453125 2.3984375 2.216796875
146 2.41658878326416 2.379999876022339 2.17578125 2.384765625 2.3984375 2.216796875
147 2.411651849746704 2.379166603088379 2.2109375 2.41796875 2.3984375 2.216796875
148 2.4061472415924072 2.3785715103149414 2.197265625 2.3984375 2.396484375 2.216796875
149 2.3872017860412598 2.378124952316284 2.203125 2.404296875 2.396484375 2.216796875
150 2.3678736686706543 2.380263090133667 2.1796875 2.390625 2.396484375 2.216796875
151 2.3650453090667725 2.383695602416992 2.208984375 2.39453125 2.396484375 2.216796875
152 2.3658950328826904 2.38611102104187 2.21875 2.3984375 2.39453125 2.216796875
153 2.3658599853515625 2.386666774749756 2.2265625 2.3828125 2.39453125 2.216796875
154 2.3673224449157715 2.385937452316284 2.220703125 2.30859375 2.392578125 2.216796875
155 2.3711612224578857 2.385294198989868 2.244140625 2.333984375 2.392578125 2.216796875
156 2.3709206581115723 2.3847222328186035 2.23828125 2.333984375 2.392578125 2.232421875
157 2.3715829849243164 2.3842105865478516 2.244140625 2.35546875 2.392578125 2.232421875
158 2.376955509185791 2.385256290435791 2.23828125 2.408203125 2.392578125 2.232421875
159 2.3813040256500244 2.3862500190734863 2.259765625 2.345703125 2.392578125 2.232421875
160 2.379300355911255 2.387195110321045 2.2421875 2.39453125 2.39453125 2.232421875
161 2.3814873695373535 2.3880953788757324 2.228515625 2.375 2.39453125 2.232421875
162 2.3860273361206055 2.389444351196289 2.236328125 2.3515625 2.39453125 2.232421875
163 2.3873162269592285 2.390625 2.2734375 2.396484375 2.39453125 2.234375
164 2.388843536376953 2.3910000324249268 2.232421875 2.3984375 2.39453125 2.234375
165 2.3785252571105957 2.3892855644226074 2.232421875 2.375 2.39453125 2.234375
166 2.373641014099121 2.3885416984558105 2.23828125 2.41796875 2.39453125 2.234375
167 2.3926665782928467 2.3880434036254883 2.24609375 2.380859375 2.39453125 2.234375
168 2.394075870513916 2.387500047683716 2.236328125 2.3984375 2.39453125 2.234375
169 2.3791630268096924 2.386904716491699 2.25390625 2.404296875 2.39453125 2.234375
170 2.3692915439605713 2.385256290435791 2.244140625 2.41015625 2.39453125 2.234375
171 2.3599393367767334 2.383108139038086 2.265625 2.408203125 2.39453125 2.234375
172 2.344076633453369 2.380714178085327 2.26171875 2.404296875 2.39453125 2.234375
173 2.3497443199157715 2.378030300140381 2.25390625 2.404296875 2.39453125 2.234375
174 2.368068218231201 2.3765625953674316 2.2421875 2.375 2.3984375 2.234375
175 2.369061231613159 2.3765625953674316 2.267578125 2.400390625 2.3984375 2.234375
176 2.3639538288116455 2.3765625953674316 2.24609375 2.39453125 2.40234375 2.234375
177 2.3720879554748535 2.3765625953674316 2.251953125 2.396484375 2.40234375 2.234375
178 2.372030735015869 2.374000072479248 2.244140625 2.390625 2.40234375 2.234375
179 2.369168758392334 2.372058868408203 2.27734375 2.423828125 2.40234375 2.234375
180 2.3766326904296875 2.371999979019165 2.25 2.4140625 2.40234375 2.234375
181 2.370382785797119 2.373936176300049 2.2734375 2.431640625 2.40234375 2.234375
182 2.3669965267181396 2.37583327293396 2.248046875 2.423828125 2.40234375 2.234375
183 2.372096300125122 2.377500057220459 2.279296875 2.419921875 2.40234375 2.248046875
184 2.378593921661377 2.379166603088379 2.27734375 2.408203125 2.41796875 2.248046875
185 2.3893110752105713 2.380833148956299 2.259765625 2.396484375 2.41796875 2.248046875
186 2.3991384506225586 2.3810343742370605 2.275390625 2.43359375 2.41796875 2.248046875
187 2.3984007835388184 2.3811402320861816 2.3125 2.41015625 2.41796875 2.248046875
188 2.4003453254699707 2.3812499046325684 2.3046875 2.412109375 2.41796875 2.248046875
189 2.407346725463867 2.3813636302948 2.29296875 2.41796875 2.41796875 2.248046875
190 2.403902530670166 2.382272720336914 2.2578125 2.421875 2.41796875 2.248046875
191 2.410402774810791 2.383333444595337 2.287109375 2.39453125 2.41796875 2.248046875
192 2.4132232666015625 2.3836538791656494 2.251953125 2.443359375 2.41796875 2.248046875
193 2.4067769050598145 2.384000062942505 2.25 2.412109375 2.41796875 2.248046875
194 2.3975887298583984 2.3843750953674316 2.2421875 2.42578125 2.41796875 2.248046875
195 2.4020886421203613 2.384782552719116 2.283203125 2.400390625 2.41796875 2.248046875
196 2.399963855743408 2.3852272033691406 2.28515625 2.408203125 2.41796875 2.248046875
197 2.390624523162842 2.384756088256836 2.2734375 2.416015625 2.41796875 2.248046875
198 2.381345272064209 2.3842105865478516 2.263671875 2.4296875 2.41796875 2.248046875
% 199 2.3655993938446045 2.3847222328186035 2.287109375 2.423828125 2.41796875 2.248046875
 }{\testdatanorm}

    \begin{axis}[
        width=5cm,
        height=4cm,
        xmax=115,xmin=25,
        ymax=2.5,ymin=1.5,
        % ymax=2.5,ymin=-1.8,
        ytick={-2,-1.5,-1, -0.5,0,0.5,1, 1.5, 2, 2.5},
        xlabel = {\small Distance along profile (m)}, 
        % grid=both,
        ylabel={\parbox{4cm}{Displacement in the \\ North/South direction (m)}},   
        y label style={yshift=-7pt, opacity=0},  
        % legend style = {at={(0,1)}, anchor=north west}, 
        legend columns=4,
        legend style={
            % cells={anchor=west},
            at={(1.5,1.25)},
            anchor=north,
            % only marks,
            /tikz/every even column/.append style={column sep=0.5cm},
            opacity=0,
            },
        ]   
        \addplot [color=white, line width=1.3, opacity=1] table [x expr={\thisrowno{0}},y expr={\thisrowno{1}}] {\testdatanorm};    
        \addplot [color=blue, line width=1.3, opacity=1] table [x expr={\thisrowno{0}},y expr={\thisrowno{1}}] {\testdatanorm};
        \addplot [color=cyan, line width=1.3, opacity=1] table [x expr={\thisrowno{0}},y expr={\thisrowno{2}}] {\testdatanorm};
        \addplot [color=gray, line width=1.3, opacity=1] table [x expr={\thisrowno{0}},y expr={\thisrowno{3}}] {\testdatanorm};
        \addplot [color=red, line width=1.3, opacity=1] table [x expr={\thisrowno{0}},y expr={\thisrowno{5}}] {\testdatanorm};
        \legend{Ours},
        % \legend{\cosicorr, \micmac, \gfn, Ours},
    \end{axis}
\end{tikzpicture}

==> fig/06_1_ir_iterations.tex <==
\setlength\tabcolsep{2pt}
\begin{tblr}{
  colspec = {X[c,0.1]X[c,h]X[c,h]X[c,h]},
  stretch = 0,
  rowsep = 1pt,
  hlines = {red5, 0pt},
  vlines = {red5, 0pt},
}
& \textbf{Reference$^\dagger$} & \textbf{\raft} & \textbf{Ours} \\
(a) & \includegraphics[width=2cm]{fig/v2/iterations/ws_sf0_s3_1.png} & \includegraphics[width=2cm]{fig/v2/iterations/ws_sf0_s3_2.png} & \includegraphics[width=2cm]{fig/v2/iterations/ws_sf0_s3_3.png} \\
(b) & \includegraphics[width=2cm]{fig/v2/iterations/sf0_s3_1.png} & \includegraphics[width=2cm]{fig/v2/iterations/sf0_s3_2.png} & \includegraphics[width=2cm]{fig/v2/iterations/sf0_s3_3.png} \\
(c) & \includegraphics[width=2cm]{fig/v2/iterations/sf0_s3_g_1.png} & \includegraphics[width=2cm]{fig/v2/iterations/sf0_s3_g_2.png} & \includegraphics[width=2cm]{fig/v2/iterations/sf0_s3_g_3.png} \\
\end{tblr}

